Vertical Symbolic Regression

Automating scientific discovery has been a grand goal of Artificial Intelligence (AI) and will bring tremendous societal impact. Learning symbolic expressions from experimental data is a vital step in AI-driven scientific discovery. Despite exciting progress, most endeavors have focused on the horizontal discovery paths, i.e., they directly search for the best expression in the full hypothesis space involving all the independent variables. Horizontal paths are challenging due to the exponentially large hypothesis space involving all the independent variables. We propose Vertical Symbolic Regression (VSR) to expedite symbolic regression. The VSR starts by fitting simple expressions involving a few independent variables under controlled experiments where the remaining variables are held constant. It then extends the expressions learned in previous rounds by adding new independent variables and using new control variable experiments allowing these variables to vary. The first few steps in vertical discovery are significantly cheaper than the horizontal path, as their search is in reduced hypothesis spaces involving a small set of variables. As a consequence, vertical discovery has the potential to supercharge state-of-the-art symbolic regression approaches in handling complex equations with many contributing factors. Theoretically, we show that the search space of VSR can be exponentially smaller than that of horizontal approaches when learning a class of expressions. Experimentally, VSR outperforms several baselines in learning symbolic expressions involving many independent variables.

==> tex/10.extra.experiment.tex <==




\begin{figure}[!ht]
    \centering
     \includegraphics[width=0.3\linewidth]{exps/nmse/inv_nv4_nt46_NMSE.noisy.pdf}
    \includegraphics[width=0.3\linewidth]{exps/nmse/inv_nv5_nt55_NMSE.noisy.pdf}
    \includegraphics[width=0.3\linewidth]{exps/nmse/inv_nv5_nt58_NMSE.noisy.pdf}
    \includegraphics[width=0.3\linewidth]{exps/nmse/inv_nv6_nt68_NMSE.noisy.pdf}
    \includegraphics[width=0.3\linewidth]{exps/nmse/inv_nv6_nt610_NMSE.noisy.pdf}
    \includegraphics[width=0.3\linewidth]{exps/nmse/sincos_nv4_nt46_NMSE.noisy.pdf}
    \includegraphics[width=0.3\linewidth]{exps/nmse/sincos_nv5_nt55_NMSE.noisy.pdf}
    \includegraphics[width=0.3\linewidth]{exps/nmse/sincos_nv5_nt58_NMSE.noisy.pdf}
    \includegraphics[width=0.3\linewidth]{exps/nmse/sincos_nv6_nt68_NMSE.noisy.pdf}
    \includegraphics[width=0.3\linewidth]{exps/nmse/sincos_nv6_nt610_NMSE.noisy.pdf}
    \includegraphics[width=0.2\linewidth]{exps/nmse/sincosinv_nv4_nt46_NMSE.noisy.pdf}
    \includegraphics[width=0.2\linewidth]{exps/nmse/sincosinv_nv5_nt55_NMSE.noisy.pdf}
    \includegraphics[width=0.2\linewidth]{exps/nmse/sincosinv_nv5_nt58_NMSE.noisy.pdf}
    \includegraphics[width=0.2\linewidth]{exps/nmse/sincosinv_nv6_nt68_NMSE.noisy.pdf}
    % \includegraphics[width=0.3\linewidth]{exps/nmse/sincosinv_nv6_nt610_NMSE.noisy.pdf}
    \caption{On selected Trigonometric \textit{noisy} datasets, quartiles of NMSE values of all the methods. }
    \label{fig:quartile-nmse-noisy-full}
\end{figure}


